Causality-based Explanation of Classification Outcomes

We propose a simple definition of an explanation for the outcome of a classifier based on concepts from causality. We compare it with previously proposed notions of explanation, and study their complexity. We conduct an experimental evaluation with two real datasets from the financial domain.

==> sec-7-experiments.tex <==

\begin{figure*}[t]
  \centering
  \includegraphics[width=.49\textwidth]{FIGS/top1-resp-credit.pdf}
  \includegraphics[width=.49\textwidth]{FIGS/top1-shap-credit.pdf}

  \vspace*{-1em}

  \caption{Distribution of the top ranked features for the (left) resp-score,
    and (right) shap-score for varying number of buckets.}
  \label{fig:top4-intersection}
\end{figure*}


\subsection{Experiments with  the Kaggle Credit Card Fraud Dataset}
\label{sec:creditcarddata}

% We next consider the Kaggle Credit Card Fraud
% dataset\footnote{https://www.kaggle.com/mlg-ulb/creditcardfraud}, which is
% used to detect fraudulent credit card transactions.

We next present our results for the evaluation of the black-box \resp\ and
\shap-scores on the Kaggle Credit Card Fraud dataset.

{\bf Classification Model.} We use as classifier a logistic regression
model. Since, the dependent variable in the dataset is highly unbalanced, we the
classifier is trained over an undersample of the training data, which has an
equal distribution of positive and negative outcomes.\footnote{Our model is
  based on the instructions in this notebook:
  https://www.kaggle.com/janiobachmann/credit-fraud-dealing-with-imbalanced-datasets}
The model is have an ROC-AUC score of 0.94 on the original test dataset and
misclassifies less than 3\% of the entities.

{\bf Score Computation.}

Need to explain:
\begin{itemize}
\item The feature are continuous variables with high precision 
\item This is a problem for the two explanation scores: (1) for \shap-score, if we condition we do not get a representative distribution, (2) for \resp-score, the individual domains are so large that it is expensive to compute
\item Our solution: bucketize the data
\item \resp-score: as number of buckets increases the time to compute increases
\item \shap-score: as number of buckets decreases the time to compute increases
\item We report on the sensitivity of the scores to the bucket size 
\end{itemize} 

{\bf Evaluation Results.}

\begin{itemize}
\item Jaccard Similarity: 0.21752786220871254
\item Mention that SHAP is not robust to the bucket size but RESP is 
\item 
\end{itemize}


\ignore {

% \section{Experiments with the Loan Dataset}
% \label{sec:loandata}

% \comlb{This section will be replaced by the computations for DA and Shapley on the Credit Card Fraud dataset.}

%  The {\em loan dataset}  is about 13 features  shown in Table \ref{tab:loan}.\ignore{\footnote{A description of the features and  the kind of data can be found at: \href{https://docs.google.com/spreadsheets/d/1u-fzB5oo_6KjOtJoF3fFdiF1OYM9xa4obSIsfKOLFc0/edit\#gid=0}{\underline{Kaggle Data}}}} It contains approximately 10K entities, of which 20\% were randomly set apart as test data. The binary classification is about the outcome variable \nit{not.fully.paid}, for which  value $1$ means the client is classified as someone who will most likely not pay the loan.

% \vspace{-9mm}
% \begin{table}[H]
% {\footnotesize
% \begin{multicols}{2}
% \begin{itemize}
% \item[0.] credit.policy
% \item[1.] purpose
% \item[2.] int.rate
% \item[3.] installment
% \item[4.] log.annual.inc
% \item[5.] dti
% \item[6.] fico
% \item[7.] days.with.cr.line
% \item[8.] revol.bal
% \item[9.] revol.util
% \item[10.] inq.last.6mths
% \item[11.] delinq.2yrs
% \item[12.] pub.rec
% \end{itemize}
% \end{multicols}} \vspace{-6mm}
% \caption{Features of the loan dataset}\label{tab:loan}\vspace{-8mm}
% \end{table}

% Features \emph{credit.policy} and \emph{purpose} are categorical, and are converted to multiple binary features, i.e. taking values $0$ or $1$, using {\em one-hot encoding}. That is, each possible value $v$ for a categorical feature $C$ gives rise to a binary feature  $F_{C,v}$, which, if evaluated on an entity $\e$,  takes value $1$ exactly when $C(\e) = v$. \ For example, the \emph{purpose} feature has 7 string values. So, one-hot encoding will replace it by a vector  with one component for each of the 7 possible values.  Depending on the value of \emph{purpose} on an entity $\e$, one-hot encoding will return ``unitary" vectors, e.g.  $[0, 1, 0, 0, 0, 0, 0]$.\footnote{The values for \emph{purpose}  are ``all\_other", ``credit\_card", ``debt\_consolidation", ``educational", 	``home\_improvement", ``major\_purchase", ``small\_business". If \emph{purpose} = ``debt\_consolidation", the  one-hot-encoded vector is $[0, 0, 1, 0, 0, 0, 0]$.} 
% \ By replacing the 2 categorical features with the 9 associated one-hot-encoding features (including 2 extra for the already binary \emph{credit.policy} feature), we end up with  20 features as inputs to a classification model.

% Notice that one-hot-encoding is used only to define and build the classification model, but is not needed for explanations or scores when the model is (or is used as) a black-box model.

% We used XGBoost to train binary classification model, with roughly 8K entities. The classifier applied to the test data, gave label $1$  to 978 entities, and label $0$ to 926 entities.
% \ The XGBoost Python library we used does not produce or show an explicit formula for the classification model. Hence, it can be considered as sufficiently ``black-box" for our purposes. However, it does identify some model's  parameters, such as their relative {\em importance}, as shown in Figure \ref{fig:weights}. Importance quantifies the relevance of a feature for the splitting points in the construction of decision trees. As such, importance is a a global measure, i.e. not associated to a particular classification.


% % \begin{figure}[H]
% %     \begin{center}\includegraphics[width=10cm]{FIGS/xgboost_feature_importances.png}
% %     \end{center}\vspace{-6mm}
% %     \caption{Feature importance scores given by the XGBoost.}\label{fig:xgb_feature_importance}
% %     \label{fig:weights}
% % \end{figure}

% In Figure \ref{fig:weights}, ``x1" stands for feature \nit{purpose}. ``x0" stands for feature \nit{credit policy}. Since they are categorical, they both give rise to one-hot-encodings. Hence, the several ``versions" of each of them, for their different values.
% \ For example, the new a binary feature { \footnotesize \verb+"one_hot_enc_x1_small_bussiness"+} is  created for the value {\footnotesize \verb+"small_business"+} of categorical feature \nit{purpose}.



% The ROC AUC (area under the curve) was computed using the ``scikitlearn" Python Library on the predictions for the test data, obtaining  0.693 of accuracy.





% \subsection{Experiments with  DA-scores}\label{sec:expsDA}

% {\em For reasons of space, in this work we show experimental results only for label $1$, which for both the loan and the FICO datasets, is the ``negative" outcome we want to explain.}\footnote{More complete experiments can be found in \cite{raiExpl}}.



% In the experiments with the DA-score we used the test data. 
% The DA-scores failed for some entities.  Similarly, for some features $F$, $\nit{da}_\e(F)=0$ for every entity $\e$.   \ In the graphs that follow, the features have been ordered on the horizontal axis according to Table \ref{tab:loan}.

% %\vspace{-1cm}
% \begin{figure}%[H]
% \begin{center}
%   %  \includegraphics[width=8cm]{FIGS/da-score-best-feature-freq-label0.png}
%     \includegraphics[width=8cm]{FIGS/da-score-best-feature-freq-label1.png}
%     \end{center}
%    \vspace{-5mm} \caption{Relative frequencies of features having highest DA-score for test entities with label $1$.}\label{fig:adj_freq}%\vspace{-20mm}
% \end{figure}

%  Figure \ref{fig:adj_freq} shows the top explanations for the entities that got label $L=1$ (out of 1904 test entities).  
% For example, for the entities with a ``bad'' outcome,  around 45\% had \nit{inq.last6mths} as top DA-score-based explanation (i.e.  highest DA-score).

% Out of the total of 1904  test entities, the actual counts for  Label 1  are: [77, 238, 0, 0, 0, 1, 0, 0, 94, 21, 365, 0, 22].  \ For  204 entities out of the 1904 in the test dataset, {\em every feature} had a  DA-score of 0. \  In particular, 44 entities with label $0$ did not exhibit any DA-best feature, i.e. for them all features have $0$ as DA-score. This situation could be somehow explained by saying that the decisions for these entities (either 0 or 1) were very robust, in that, changing any single feature, did not change the outcome.
  
% We should note that three of the features with highest  DA-scores  have small domains (as based on the test data). We recall that \nit{credit.policy} and \nit{purpose} have two and seven possible values, respectively, while \nit{inq.last.6mths} has 34  possible values. However,  a small domain does not guarantee a large DA-score. For example, \nit{delinq.2yrs} has 14 possible values, and its DA-score is 0 for most entities, but it takes twice the highest DA-score for an entity.


% \begin{figure}%[H]
% \begin{center}
%   \includegraphics[width=8.5cm]{FIGS/shapley-best-feature-freq-label1.png}
%     \end{center}
%   \caption{Relative frequency with which each feature has the highest Shapley-score test entities  classified as  1. }\label{fig:adj_freq_shap}
% \end{figure}

% \subsection{Experiments with Shapley-scores}\label{sec:expsShap}



% We now report on experiments with an exact computation of the Shapley-score on the loan data  (experiments with the  Banzhaf-score are shown in \cite{raiExpl}). 

% The results in Figure \ref{fig:adj_freq_shap} are for the  1024 entities in the same test set  used in the previous section, with all features considered.  For the test entities with label $1$, the actual counts for features as the highest according to the Shapley-score are:  {\footnotesize [0, 180, 0, 292, 3, 1, 319, 26, 138, 0, 0, 308, 120]}. 






% \begin{figure}[H]
%   \begin{center}  
%         \includegraphics[width=9cm]{FIGS/shapley-best-feature-freq-label1-avg.png}
%     \end{center}
%    \caption{Relative averaged frequency with which each feature has the highest Shapley-score for test entities classified as 1. }\label{fig:avg_freq_shap}
% \end{figure}

% For some entities there are two or more features that have the same  maximum Shapley score. A possible ways to resolve ties is as shown in Figure \ref{fig:adj_freq_shap}, where we assume every feature with the maximum score represents an explanation for that entity; thus, some entities have more than one explanation, and the  relative frequencies may  add up to more than 1. \
% An alternative is to resolve the tie by dividing the weight among the $k$ features with the maximum score, i.e.  each contributes $\frac{1}{k}$ to the count. In this way we obtain Figure \ref{fig:avg_freq_shap},  displaying {\em averaged frequencies}, with weights adding up to  1. 
% The counts for this graph  are: \ {\footnotesize $[0, 53.67, 0, 127.27, 0.53, 0.17, 141.30, 7.67, 47.47, 0, 0,$ $ 111.72, 31.22]$}.  


% \subsection{Comparing DA and Shapley   Scores}\label{sec:1stComp}

% Now we make some comparisons between DA- and Shapley-scores for the loan data, exact Shapley-scores are exact and including all 13 features. \ Figures \ref{fig:adj_freq} and \ref{fig:avg_freq_shap} show that the alignment of DA- and Shapley-scores is not perfect.  In Figure \ref{fig:adj_freq}, most top DA-scores correspond to feature \nit{inq.last.6mths}, which almost never appears with the top Shapley-score.  Only \nit{purpose} and \nit{revol.bal} seem to have somewhat similar frequencies as top DA-scores or as top Shapley-scores.




% For a deeper understanding,  Figures \ref{fig:compare_da_shap_0_1} and \ref{fig:compare_da_shap_1_1},
% show  a  closer comparison between DA- and Shapley-scores. In each of them the horizontal axis shows the 13 possible {\em positions} (or ranks) of features determined by a score (DA or Shapley), starting from 0; i.e. the feature with the highest DA- or Shapley-score has rank 0, the next has rank 1, etc. 

% \begin{figure}[H]
% \begin{center}
%     \includegraphics[width=8.5cm]{FIGS/da-choosing-best-shapley-pos-0-label-1.png}
  
%     \includegraphics[width=8.5cm]{FIGS/shapley-choosing-best-da-pos-0-label-1.png}
%     \end{center}
%    \caption{For test entities with label 1.  Top: Number of times the $i$th DA-top  feature  is also Shapley-top. \ Bottom: Number of times the $i$th Shapley-top  feature is also DA-top. }\label{fig:compare_da_shap_0_1}
% \end{figure}


% Figure \ref{fig:compare_da_shap_0_1}, bottom, shows, for each DA-rank $i$ the number of times  it occurs with top Shapley-score, i.e. has Shapley-rank 0. All this for the test entities  classified with label $1$. That is,  all possible DA-ranks, from $0$ to $12$, are contrasted with Shapley-rank $0$. 
% \
% More precisely, the graph in Figure \ref{fig:compare_da_shap_0_1}, bottom, is generated as follows: \ (a)
%      For each test entity, take the most important feature determined by the Shapley-score. \ (b) 
%      If the feature is the $i$th most important feature chosen by the DA-score for the same record, increment by one counter for position $i$.
     

 
% For example, in the highest bar in  Figure \ref{fig:compare_da_shap_0_1}, top, shows that for 12 entities, the top DA-score corresponds to the feature that has Shapley-rank $i=2$  (i.e. third position).  \ For the same figure, bottom, around 230 times the 9th DA-ranked feature is chosen as the top Shapley-score feature. \ For the graph at the top, the scores are swapped, i.e. the top DA-rank is compared with all possible Shapley-ranks, appearing in the horizontal axis.  \ Similarly, Figure  \ref{fig:compare_da_shap_1_1}, top, the second-top DA, i.e. DA-position 1, is compared with all features along the Shapley-ranking. And the other way around in the same figure, bottom.


% \begin{figure}[H]
% \begin{center}
%     \includegraphics[width=8.5cm]{FIGS/da-choosing-second-shapley-label-1.png}
    
%     \includegraphics[width=8.5cm]{FIGS/shapley-choosing-second-da-label-1.png}
%     \end{center}
%    \caption{For test entities with label 1. Top: Number of times the $i$th DA-top  feature  is also second-top Shapley. Bottom: Number of times the $i$th Shapley-top  feature  is also second-top DA.} \label{fig:compare_da_shap_1_1}
% \end{figure}

% \red{The counts for the graphs on the left are lower since the DA-score is more likely to give a record-feature pair a score of 0, which is ignored by the counter.}


}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "deemScores"
%%% End:

